The Mathematical Foundations of Manifold Learning

Manifold learning is a popular and quickly-growing subfield of machine learning based on the assumption that one's observed data lie on a low-dimensional manifold embedded in a higher-dimensional space. This thesis presents a mathematical perspective on manifold learning, delving into the intersection of kernel learning, spectral graph theory, and differential geometry. Emphasis is placed on the remarkable interplay between graphs and manifolds, which forms the foundation for the widely-used technique of manifold regularization. This work is written to be accessible to a broad mathematical audience, including machine learning researchers and practitioners interested in understanding the theorems underlying popular manifold learning algorithms and dimensionality reduction techniques.

==> chapters/__latexindent_temp.tex <==
\chapter{Foundations} \label{chap:foundations}

The first step in understanding machine learning algorithms is to define our learning problem. 
In this chapter, we will only work in the supervised setting, generally following the approaches from \cite{mitnotes,shalev2014understanding,castro20182di70}. \autoref{chap:manireg} will extend the framework developed here to a semi-supervised setting. 

% This chapter generally follows the approach laid out in 

% A learner aims to estimate a function $f: X \to Y$, where $X$ is denoted the input space and $Y$ is denoted the output space, from a finite set of data $S$. When $Y = \R$, the task is usually referred to as a type of regression, and when $Y = \fC$, it is usually referred to as a type of classification. 

% In the supervised setting, our data takes the form of paired input and output examples: $S = \{(x_i, y_i)\}_{i=1}^N$, where $x_i \in X$ and $y_i \in Y$. In the semi-supervised setting, with $l$ labeled examples and $u$ unlabeled examples, $S=\{(x_i, y_i)\}_{i=1}^l \cup \{x_i\}_{i=1}^u$. Finally, in the unsupervised setting, with only unlabeled examples, $S = \{x_i\}_{i=1}^N$. 

% In this chapter, we will only work in the supervised setting. \autoref{chap:manireg} will extend the framework developed here to an unsupervised setting. 

\subsection{Learning Algorithms \& Loss Functions}

A learning algorithm $\fA$ is a map from a finite dataset $S$ to a candidate function $\hat{f}$, where $\hat{f}$ is measurable. Note that $\fA$ is stochastic because the data $S$ is a random variable. We assume that our data $(x_i, y_i)$ are drawn independently and identically distributed from a probability space $X \times Y$ with measure $\rho$. 

We define what it means to ``do well'' on a task by introducing a loss function, a measurable function $L: X \times Y \times F \to [0, \infty)$. This loss almost always takes the form $L(x,y,f) = L'(y, f(x))$ for some function $L'$, so we will write the loss in this way moving foward. Intuitively, we should think of $L(y, \hat{f}(x))$ as measuring how costly it is to make a prediction $\hat{f}(x)$ if the true label for $x$ is $y$. If we predict $f(x) = y$, which is to say our prediction at $x$ is perfect, we would expect to incur no loss at $x$ (i.e. $L(y, \hat{f}(x)) = 0$). 

Choosing an appropriate loss function is an important part of using machine learning in practice. Below, we give examples of tasks with different data spaces $X, Y$ and different loss functions $L$.
% Common loss functions are also shown in Table %reff{}
% IFTIME: Add table of common loss functions: lsq, cosine, huber, softmax, hinge
    
\paragraph{Example: Image Classification}
Image classification, the task of classifying an image $x$ into one of $C$ possible categories, is perhaps the most widely-studied problem in computer vision. Here $x \in R^{H \times W \times 3}$, where $H$ and $W$ are the image height and width, and $3$ corresponds to the three color channels (red, green, and blue). Our label space is a finite set $Y = \fC$ where $|\fC| = C$. A classification model outputs a discrete distribution $f(x_i) = p = (p_1, \dots, p_C)$ over classes, with $p_c$ corresponding to the probability that the input image $x$ has class $c$. \\

As our loss function, we use cross-entropy loss: 
\[ L(y, f(x)) = -\frac{1}{N} \sum_{c=1}^C \ind\{y_i = c\} \log(p_c), \quad p = f(x_i) \]

\paragraph{Example: Semantic Segmentation}
As mentioned in the introduction, semantic segmentation is the task of classifying every pixel in an input image. Here, $X = \fC^{H \times W \times 3}$ like in image classification above, 
% \footnote{In semantic segmentation it is also common to use RGBD image inputs, in which case $x$ would have $4$ channels (red, green, blue, depth).} 
but $Y = \fC^{H \times W}$ unlike above. The output $f(x) = p = (p_{c}^{(h,w)})$ is a distribution over classes for each pixel. \\

As our loss function, we use cross-entopy loss averaged across pixels: 
\[ \hspace*{-3pt} L(y, f(x)) = -\frac{1}{N\cdot H\cdot W}  \sum_{h=1}^H \sum_{w=1}^W  \sum_{c=1}^C 1\{y_i^{(h,w)} = c\} \log(p_c^{(h,w)}), \quad p = f(x_i^{(h,w)}) \]

\paragraph{Example: Crystal Property Prediction}
A common task in materials science is to predict the properties of a crystal (e.g. formation energy) from its atomic structure (an undirected graph). As a learning problem, this is a regression problem with $X$ as the set of undirected graphs and $Y=\R$. \\

For the loss function, it is common to use mean absolute error (MAE) due to its robustness to outliers:
\[ L(y, f(x)) = |y - f(x)|\]

\section{The Learning Problem}

Learning is about finding a function $\hat{f}$ that generalizes from our finite data $S$ to the infinite space $X \times Y$. This idea may be expressed as minimizing the expected loss $\fE$, also called the risk: 
\[ \fE(f) = \E[L(y, f(x))] = \int_{X \times Y} L(y, f(x)) \, d\rho(x,y) \]
Our objective in learning is to minimize the risk: 
\[ f^{*} = \argmin_{f \in \fF} \E[L(y, f(x))] = \argmin_{f \in \fF} \int_{X \times Y} L(y, f(x)) \, d\rho(x,y) \]
Since we have finite data, even computing the risk is impossible. Instead, we approximate it using our data, producing the empirical risk: 
\begin{equation} \label{eq:erm}
\fhE(f) = \frac1n \sum_{i=1}^N L(y_i, f(x_i)) \approx \int_{X \times Y} L(y, f(x)) \, d\rho(x,y)
\end{equation}
This concept, \textit{empirical risk minimization}, is the basis of much of modern machine learning. 

One might hope that by minimizing the empirical risk over all measurable functions, we would be able to approximate the term on the right hand side of \ref{eq:erm} and find a function $\hat{f} = \argmin_{f \in \fF}\fhE(f)$ resembling the desired function $f^*$. However, without additional assumptions or priors, this is not possible. In this unconstrained setting, no model can achieve low error across all data distributions, a result known as the No Free Lunch Theorem. 

The difference between the performance of our empirically learned function $\hat{f}$ and the best possible function is called the generalization gap or generalization error. We aim to minimize the probability that this error exceeds $\ep$: 
\[ \P\l \fE(\hat{f}) - \inf_{f \in \fF}\fE(f) > \ep \r \]
Note that here $\P$ refers to the measure $\rho^N$ and that $\hf$ is a random variable because it is the output of $A$ with random variable input $S$.\footnote{Technically $\fA$ could also be random, but for simplicity we will only consider deterministic $A$ and random $S$ here.} 

It would be desirable if this gap were to shrink to zero in the limit of infinite data: 
\begin{equation} \label{eq:consistency} 
    \lim_{n\to\infty} \P \l  \fE(\hat{f}) - \inf_{f \in \fF}\fE(f) > \ep  \r = 0 \qquad \forall \ep > 0
\end{equation}
A learning algorithm with this property is called \textit{consistent} with respect to $\rho$. Stronger, if property \ref{eq:consistency} holds for all fixed distributions $\rho$, the algorithm is \textit{universally consistent}. Even stronger still, an algorithm that is consistent across finite samples from all distributions is \textit{uniformly universally consistent}:
\begin{equation} \label{eq:univconsistency} 
\lim_{n\to\infty} \sup_\rho \P\l \fE(\hat{f}) - \inf_{f \in \fF}\fE(f) > \ep \r = 0 \qquad \forall \ep > 0
\end{equation}

Unfortunately, this last condition is \textit{too} strong. This is the famous ``No Free Lunch'' Theorem. 

\begin{theorem}[No Free Lunch Theorem] \label{thm:nofreelunch}
    No learning algorithm achieves uniform universal consistency. That is, for all $\ep > 0$: 
    \[ \lim_{n\to\infty} \sup_\rho \P\l \fE(\hat{f}) - \inf_{f \in \fF}\fE(f) > \ep \r = \infty \]
\end{theorem}
% We include a proof of this result for binary classification in Appendix \ref{appendix:nfl}. 
For a simple proof, the reader is encouraged to see \cite{shalev2014understanding} (Section 5.1). 

\section{Regularization}

The No Free Lunch Theorem states that learning in an entirely unconstrained setting is impossible. Nonetheless, if we constrain our problem, we can make meaningful statements about our ability to learn. 

Looking at Equation \ref{eq:univconsistency}, there are two clear ways to constrain the learning problem: (1) restrict ourselves to a class of probability distributions, replacing $\sup_{\rho}$ with $\sup_{\rho \in \Theta}$, or (2) restrict ourselves to a limited class of target functions $\fH$, replacing $\inf_{f \in \fF}$ with $\inf_{f \in \fH}$. We examine the latter approach, as is common in statistical learning theory.

To make learning tractable, we optimize over a restricted set of hypotheses $\fH$. But how should we choose $\fH$? On the one hand, we would like $\fH$ to be large, so that we can learn complex functions. On the other hand, with large $\fH$, we will find complex functions that fit our training data but do not generalize to new data, a concept known as \textit{overfitting}.

% IFTIME: Add Figure of overfitting and underfitting 

Ideally, we would like to be able to learn complex functions when we have a lot of data, but prefer simpler functions to more complex ones when we have little data. We introduce \textit{regularization} for precisely this purpose. Regularization takes the form of a penalty $R$ added to our loss term, biasing learning toward simpler and smoother functions. 

Most of this thesis is concerned with the question of what it means to be a ``simple'' or ``smooth'' function. Once we can express and compute what it means to be simple or smooth, we can add this as a regularization term to our loss. 

Moreover, if we have any tasks or problem-specific notions of what it means to be a simple function, we can incorporate them into our learning setup as regularization terms. In this way, we can inject into our algorithm prior knowledge about the problem's structure, enabling more effective learning from smaller datasets. 

With regularization, learning problem turns into:
\[ \arg\min_{f \in \fH }  \fhE(f, x, y) + \lam R(f, x, y) \]
where $\fH$ can be a relatively large hypothesis space. 

The parameter $\lam$ balances our empirical risk term and our regularization term. When $\lam$ is large, the objective is dominated by the regularization term, meaning that simple functions are preferred over ones that better fit the data. When $\lam$ is small, the objective is dominated by the empirical risk term, so functions with lower empirical risk are preferred even when they are complex. Tuning $\lam$ is an important element of many practical machine learning problems, and there is a large literature around automatic selection of $\lam$ \cite{abdessalem2017automatic}. 

\textit{Notation: } The full expression $L + \lam R$ is often called the loss function and denoted by the letter $L$. We will clarify notation in the following chapters whenever it may be ambiguous. 

Often, $R$ depends only on the function $f$ and its parameters. We will call this data-independent regularization and write $R(f)$ for ease of notation. The reader may be familiar with common regularization functions (e.g. L1/L2 weight penalties), nearly all of which are data-independent. Manifold regularization, explored in \autoref{chap:manireg}, is an example of data-dependent regularization. 

\paragraph{Example (Data-Independent): Linear Regression} 
In linear regression, it is common to add a regularization term based on the magnitude of the weights to the standard least-squares objective: 
\[ R(f) = ||w||^\al \text{ for $\al > 0$ }\]
When $\al = 2$, this is denoted Ridge Regression, and when $\al = 1$, it is denoted Lasso Regression. Both of these are instances of Tikhonov regularization, a data-independent regularization method explored in the following chapter. 

\paragraph{Example (Data-Dependent): Image Classification}
When dealing with specialized domains such as images, we can incorporate additional inductive biases into our regularization framework. For example, we would expect an image to be classified in the same category regardless of whether it is rotated slightly, cropped, or flipped along a vertical line. \\

Recent work in visual representation learning employs these transformations to define new regularization functions. For example, \cite{xie2019unsupervised} introduces a 
% self-supervised 
% we could add a 
regularization term penalizing the difference between a function's predictions on an image and an augmented version of the same image: 
\[ R(f, x) = KL(f(x), f(\text{Aug}(x)) \]
where $\text{Aug}$ is an augmentation function, such as rotation by $15^{\circ}$, and $KL(\cdot, \cdot)$ is the Kullback–Leibler divergence, a measure of the distance between two distributions (because $f(x)$ is a distribution over $C$ possible classes). This method currently gives state-of-the-art performance on image classification in settings with small amounts of labeled data \cite{xie2019unsupervised}.


==> frontmatter/__latexindent_temp.tex <==

This is an edited version of my undergraduate thesis, submitted to the Harvard Math Department in May 2020. It differs from the original thesis in one major respect, namely that this version omits the proofs of a number of theorems that are readily-available in other expositions. Whereas the original version reproduced these proofs in full, this version simply contains references to these proofs in other works.
% This is an edited version of an undergraduate thesis submitted to the Harvard Mathematics Department. It differs from the original thesis in one major respect, namely that this version omits the proofs of a number of theorems that are readily-available in other expositions. Whereas the original version reproduced these proofs in full, this version simply contains references to these proofs in other works.

This thesis is built upon an extensive body of prior work in learning theory, graph theory, differential geometry, and manifold learning. In particular, I would like to thank \hyperlink{cite.mitnotes}{Professors Lorenzo Rosasco and Tomaso Poggio} for their lectures on statistical learning theory, \hyperlink{cite.spielman2007spectral}{Professor Daniel Spielman} for his notes on spectral graph theory, \hyperlink{cite.canzani2013analysis}{Professor Yaiza Canzani} for her notes on analysis on manifolds, and \hyperlink{cite.belkin2006manifold}{Professor Mikhail Belkin} for his work on manifold learning.

Finally, I wish to thank those people without whom I could never have written this thesis: my family, friends, and wonderful advisor \hyperlink{http://www.childrenshospital.org/research/researchers/m/arjun-manrai}{Raj}. Unlike the manifolds discussed herein, their support was truly boundless. 

I hope you enjoy and learn something from this thesis! If you have comments, corrections, or would like to contact me for anything else, feel free to \hyperlink{luke.melas@gmail.com}{email me}. 

- Luke

==> frontmatter/authorlist.tex <==
\noindent The following authors contributed to Chapter 1: Albert Einstein, George Gamow and Pief Panofsky.

\noindent The following authors contributed to Chapter 2: I. I. Rabi, Niels Bohr and Norman Ramsey.

\noindent The following authors contributed to Chapter 3: Ramon y Cajal, Andrew Huxley. 


==> frontmatter/authorsnote.tex <==

This is an edited version of my undergraduate thesis, submitted to the Harvard Mathematics Department in May 2020. It differs from the original thesis in one major respect, namely that this version omits the proofs of a number of theorems that are readily-available in other expositions. Whereas the original version reproduced these proofs in full, this version simply contains references to these proofs in other works.
% This is an edited version of an undergraduate thesis submitted to the Harvard Mathematics Department. It differs from the original thesis in one major respect, namely that this version omits the proofs of a number of theorems that are readily-available in other expositions. Whereas the original version reproduced these proofs in full, this version simply contains references to these proofs in other works.

This thesis is built upon an extensive body of prior work in learning theory, graph theory, differential geometry, and manifold learning. In particular, I would like to thank \hyperlink{cite.mitnotes}{Professors Lorenzo Rosasco and Tomaso Poggio} for their lectures on statistical learning theory, \hyperlink{cite.spielman2007spectral}{Professor Daniel Spielman} for his notes on spectral graph theory, \hyperlink{cite.canzani2013analysis}{Professor Yaiza Canzani} for her notes on analysis on manifolds, and \hyperlink{cite.belkin2006manifold}{Professor Mikhail Belkin} for his work on manifold learning.

Finally, I wish to thank those people without whom I could never have written this thesis: my family, friends, and wonderful advisor \hyperlink{http://www.childrenshospital.org/research/researchers/m/arjun-manrai}{Professor Arjun Manrai}. Unlike the manifolds discussed herein, their support was truly boundless. 

I hope you enjoy and learn something from this thesis! If you have comments, corrections, or would like to contact me for anything else, feel free to \hyperlink{luke.melas@gmail.com}{email me}. 

 - Luke

==> frontmatter/dedication.tex <==
% This document is an edited version of an undergraduate thesis submitted to the Harvard Mathematics Department. It differs from the original thesis in that this version omits the proofs of a number of theorems that are readily-available in the literature. Whereas the original version reproduced these proofs in full, this version simply contains references that show where the reader may find these proofs. 

% This thesis is built upon an extensive body of prior work in learning theory, spectral graph theory, differential geometry, and manifold learning. 

% In particular, I would like to thank \citeauthor{mitnotes} for his 





% Finally, I wish to thank those people without whom this would not have been possible: my family, my friends, and my wonderful advisor Raj. Unlike the manifolds discussed herein, their support was truly boundless. 


==> frontmatter/thanks.tex <==
% ORIGINAL: % I wish to thank my family, my friends, and my wonderful advisor Professor Arjun Manrai for their support throughout this process.

% NEW: % I wish to thank my family, my friends, and my wonderful advisor Raj. Unlike the manifolds discussed herein, their support was truly boundless. 
